Artiverse: A Diverse and Physically Grounded Dataset for Articulated Objects

We present Artiverse, a diverse and physically grounded dataset of high-quality articulated 3D objects designed for realistic functional modeling and simulation. Artiverse contains 5.4K human-authored objects across a broad range of 88 categories, aggregated from multiple 3D static repositories. Objects are annotated with functional parts, interior structures, realistic kinematic relationships and articulated joints including multi-DoF joints, and physical attributes such as metric scale, material, and mass. We develop a semi-automated annotation pipeline that combines few-shot segmentation, geometric reasoning, and multi-stage human verification to achieve high-quality and efficient annotation, reducing manual annotation time by over 30%. We demonstrate the value of Artiverse on tasks of part mobility analysis, articulated object generation, and physics-based interaction. Artiverse provides a data resource to advance functional understanding for articulated objects.

==> figures/annotation_representation.tex <==
\begin{figure*}[t]
\centering
\includegraphics[width=\linewidth]{visuals/annotation_rep.pdf}
\caption{Annotation illustration with an example data in Artiverse. 
\TODO{Replace the renderings}
}
\label{fig:annotation_rep}
\vspace{1em}
\end{figure*}

==> figures/articulation.tex <==
\begin{figure}[t]
\centering
\includegraphics[width=\linewidth]{example-image}
\caption{
Outline of the articulation module. \todo{Replace 2 with section number, recolor the arrows}
} 
\label{fig:articulation}
\end{figure}

==> figures/articulation_heuristics.tex <==
\begin{figure}[t]
\centering
\includegraphics[width=\linewidth]{example-image}
\caption{
Visualization of articulation heuristics examples.
} 
\label{fig:articulation_heuristics}
\end{figure}

==> figures/articulation_ranges.tex <==
\begin{figure}[t]
\centering
\includegraphics[width=\linewidth]{example-image}
\caption{
Visualization of articulation heuristics examples.
} 
\label{fig:articulation_ranges}
\end{figure}

==> figures/interior_completion.tex <==
\begin{figure}[t]
\centering
\includegraphics[width=\linewidth]{example-image}
\caption{
Outline of the interior completion module.
} 
\label{fig:int_comp}
\end{figure}

==> figures/obj_examples.tex <==
\begin{figure}[h]
\centering
\vspace{-3mm}
\includegraphics[width=\linewidth]{visuals/objs.png}
\vspace{-10mm}
\label{fig:objs}
\end{figure}

==> figures/preprocesing.tex <==
\begin{figure}[t]
\centering
\includegraphics[width=\linewidth]{visuals/preprocessing_module.pdf}
\caption{
Outline of the preprocessing module. \todo{Replace 0 with section number}
\Ali{The figure should be redesigned, it is too small and the space is not utilized well. }} 
\label{fig:preprocesing}
\end{figure}

==> figures/segmentation.tex <==
\begin{figure}[t]
\centering
\includegraphics[width=\linewidth]{visuals/segmentation_module.pdf}
\caption{
Outline of the segmentation module. 
\TODO{Figure redesign: replace 1 with section number, recolor the arrows, change SOFA to ASIA}
% \todo{Replace 1 with section number, recolor the arrows}
% \Ali{SOFA should be ASIA}
} 
\label{fig:segmentation}
\end{figure}

==> sec/legacy_3_dataset.tex <==
\section{Artiverse}
\input{figures/pipeline_overview}

\subsection{Design Principles}
\label{subsec: design_principles}
% \AXC{most of this paragraph should go into section 4.  This paragraph should start with design principles (see comment for section 3.1)}  
The construction of Artiverse is guided by five design principles that shape both the annotation framework and the underlying data structure.
They ensure that the dataset is comprehensive, consistent, and scalable for studying functional articulated object behavior.

\mypara{Object coverage.}
Artiverse focuses on human-made, everyday objects that exhibit articulation and afford interaction, such as furniture, tools, and appliances.
We prioritize categories that appear frequently in human environment (e.g., household, office, and outdoor) to ensure relevance for real-world applications.
We organize the objects in three levels of semantic categories: super-category, main category, and sub-category.
The super-categories are designed to be broad and general (e.g., appliance, lighting, kitchenware), the main categories are specific to the object function (e.g., toaster, window, dispenser), and the sub-categories capture fine-grained distinctions in the usage context (e.g, office chair vs. bar stool, trash can vs. dumpster). 
The category labels are following WordNetCo used in HSSD dataset~\cite{khanna2024habitat} with a few labels expanded for new sub-categories.

\mypara{Part granularity.}
We define a unified taxonomy of functionally informed part labels that capture both articulated components and their assoicated interaction affordance regions (e.g., handles, backrest).
These labels are designed to be semantically meaningful across categories, enabling models to generalize functionality understanding beyond category boundaries.

\mypara{Annotation consistency.}
To maintain coherent semantics across large-scale data, we use category-level templates that specify the expected part structures and possible motion types for each object family.
These templates guide both automated inference and human verification, ensuring consistent labeling and complete articulation coverage across the dataset.

\mypara{Scalability of annotation process.}
We design a semi-automated annotation workflow that integrates few-shot segmentation, VLM inference, and geometric heuristics to efficiently generate initial proposals, followed by multi-stage human verification.
This design reduces manual effort while maintaining accuracy, enabling us to scale annotation to thousands of raw or partially labeled static models.

\mypara{Standardization across data sources.}
Since our assets are aggregated from multiple repositories, we enforce standardized orientation, metric scale, texture fidelity, and mesh quality, along with a unified data and annotation schema.
Each object is associated with metadata that records its unique UUID, source dataset, original model ID, and category labels to ensure traceability and reproducibility.

% Artiverse collects human-made articulated objects from multiple 3D repositories (see data sources in \Cref{tab:ds_compare}).
% To scale up the process of model selection and annotation, we design a semi-automated framework that combines human expertise and algorithmic assistance to efficiently produce high-quality data.
% Our data construction framework consists of three key modules as model collection, annotation, and assets standardization, as shown in \Cref{fig:pipeline-overview}.
% We leverage recent advances in VLMs and vision foundation models, combined with heuristic-based algorithms to initiate data selection and annotation proposals across different modules.
% Human experts then refine and verify these proposals through web-based interfaces to ensure all the annotations are accurate and consistent.
% In the following sections, we will illustrate how we organize our data (in \Cref{subsec:dataset_design}), what attributes are annotated (in \Cref{subsec:annotation}), and how we design each module in the semi-automated framework (in \Cref{sec:framework})
% to construct Artiverse in detail.

% \di{Artiverse is a dataset of articulated 3D shapes that are sourced from existing, non-articulated datasets. 
% We design a semi-automated pipeline to facilitate efficient annotation, in the core of which are: propagation of annotations from examples and the usage of the generalizable geometric heuristics. 
% The following subsections discuss our dataset creation process in detail. } 
% \Ali{Can you sxhow a pipe-line abstraction of the whole process?}
% \todo{There should be an overview diagram of the main components of the system}

\subsection{Dataset Structure}
\label{subsec:dataset_design}

% \AXC{What follows is not a set of design principles but just description of the characteristics of the dataset.  The design principles should cover both the design of the annotation framework as well as the data structure and should be pulled up.   Design principles would be: 1) semi-automated workflow for efficient annotation (I'm not sure we actually achieve the efficient annotation part), 2) something about the types of objects and categorization and part labels we choose to focus on: can be broad-coverage of common objects that people interact with or functional informed part labels, 3)... }

% \mypara{Object categorization.}
% We organize the objects in three levels of semantic categories: super-category, main category, and sub-category.
% The super-categories are designed to be broad and general (e.g., appliance, lighting, kitchenware), the main categories are specific to the object function (e.g., toaster, window, dispenser), and the sub-categories capture fine-grained distinctions in the usage context (e.g, office chair vs. bar stool, trash can vs. dumpster). 
% The category labels are following WordNetCo used in HSSD dataset~\cite{khanna2024habitat} with a few labels expanded for new sub-categories.

\mypara{Per-category templates.}
We maintain a template for each object main category.
Each template enumerates all possible parts with standardized semantic labels, organized in a two-level hierarchy: the articulated parts in the top-level and their associated affordance parts of human interaction in the second-level.
For each articulated part, the template specifies the admissible motion types, kinematic dependency with other parts (e.g., a door linked to its frame), and the possible logic chain of reactions (e.g., lifting the chair lever raises or lowers the seat) as joint dependencies.
For each interaction affordance part, the template labels the possible types of human-to-object interaction (e.g., a botton can be pushed, a seat can be sat on).
Templates are designed and verified by human experts with domain knowledge before the annotation stage, and serve the following purposes:
1) to pre-define the part labels so that the parts can be consistently segmented and labeled;
2) to provide prior knowledge to design heuristics for motion annotation and assist the kinematic graph construction;
3) to guide the human annotators to ensure the completeness and consistency for verification and refinement.

\mypara{Data representation.}
Each object is stored as a textured mesh with all the annotations embedded in a hierarchical structure, supporting three complementary formats: \textit{GLB}, \textit{USD}, and \textit{URDF}.
The GLB format is used for visualization and rendering, the USD and URDF format ensure interoperability with physics-based simulators and animation pipelines.
% Associated metadata is stored in JSON files, providing easy access to object-level information such as identifiers, category labels, and physical parameters.

% \di{Our dataset contains \todo{xxx} categories, offering a fine-grained binning of objects based on the type and functionality. For instance, each category (i.e., bookcase) falls under less functionality-specific main category (i.e., cabinet), with the final super category grouping being the most general (i.e., storage\_furniture). We provide a total of \todo{xxx} main and \todo{xxx} super categories. 
% A core part of our pipeline are templates. For each category, we develop a template that contains the parts we distinguish (both affordance- and articulated-level), their possible motion types and semantic labels of potential parents. Additionally, we supply a description of each category and each part in a template. Templates are used in design and as inputs to heuristics across the pipeline.}


% \subsection{Annotations}
% \label{subsec:annotation}
% \jy{TODO: list all the annotations that are provided in the dataset with a short description. A table might be useful here.}


% \di{For each object, we annotate the articulated parts as well as the parts related to human affordances (i.e., handles, seats, etc.). Artiverse features a total of \todo{xxx} parts across \todo{xxx} part labels. \Ali{Another table that summarizes all the aspects of artiverse might be useful here.}

% In order to obtain articulated joints, we attach the motion type to each part out of: \{\texttt{fixed}, \texttt{free}, \texttt{prismatic}, \texttt{revolute}, \texttt{continuous}, \texttt{cylindrical}, \texttt{screw}, \texttt{universal}\} as well as corresponding axes, origins and ranges as applicable.
% Finally, we infer the material label that contributes the most to the mass of each part. Which, in turn, allows us to infer masses.
% }





==> sec/legacy_4_pipeline.tex <==
\section{Semi-automated Annotation Pipeline}
\label{sec:framework}

\subsection{Overview}
Artiverse collects human-made articulated objects from multiple 3D repositories.
To scale up the process of model selection and annotation, we design a semi-automated pipeline that combines human expertise and algorithmic assistance to efficiently produce high-quality data.
We leverage recent advances in VLMs and vision foundation models, combined with heuristic-based algorithms to initiate data selection and annotation proposals across different modules.
Human experts then refine and verify these proposals through web-based interfaces to ensure all the annotations are accurate and consistent.
As shown in \Cref{fig:pipeline-overview}, our data construction framework consists of six key modules: model section and pre-processing, part segmentation, interior completion, motion annotation, physical properties estimation, and multi-stage human verification in between.
In the following sections, we will illustrate how we design each module to construct Artiverse in detail.


\input{figures/annotation_representation.tex}

\subsection{Model Selection and Pre-processing}
To construct Artiverse, we begin by defining a list of target object categories that encompass common articulated objects.
For each category, human experts first identify a few representative models within its subcategories to serve as \textit{anchors}, establishing reference exemplars for subsequent retrieval.
We then use a two-stage retrieval strategy that combines metadata filtering and visual embedding similarity to collect shapes from the model pool.
Since the level of metadata detail varies across repositories, we first perform coarse filtering through text-based matching to exclude irrelevant objects.
Next, we apply fine-grained visual retrieval using DuoduoCLIP~\cite{lee2025duoduo} features: multi-view turntable renderings are generated for each candidate model, and feature similarities are computed against the anchor exemplars.
A custom web interface is used to review and verify the top-$k$ retrieved candidates, from which we retain models that match the intended category and exhibit realistic geometry and textures.
The resulting collection forms the initial pool of high-quality candidate models for downstreaming annotation.
Before pass into the following stages of the pipeline, we ensure the consistent orientation and physical size is determined either coming with the data source or estimated by VLMs.

% \di{The first module of our pipeline is a pre-processing module, outlined in ~\Cref{fig:preprocesing}. \Ali{this sentence is too small to be a separate paragraph. You need to explain what is being fed to this step and what is being sent out. Why we need this step in a high level.  }
% The process begins with \Ali{the selection of} the shapes using the UI. We leverage existing UI from SSTK\footnote{\url{https://github.com/smartscenes/sstk}} (the Model Viewer Interface), that allows to search across many datasets of interest, with exception of Objaverse and TexVerse \Ali{why this exception?}. In particular, we enter the category name as a search query and the search is conducted on the shape descriptions and category labels from source datasets.
% As Objaverse provides neither the descriptions nor labels, we employ a different strategy by leveraging the learned embeddings for search. More specifically, after conducting non-Objaverse search, we select the representative shapes from each category using K-means and compute DuoDuoCLIP~\cite{lee2025duoduo} embeddings using the multi-view renderings. Finally, we use these embeddings to query the set of precomputed embeddings from Objaverse and conduct selection out of the most similar shapes.
% After selecting the shapes, we design the template by organizing articulated and affordance-related parts we encountered, their possible articulations, and parent-child relationships. In fact, our templates define the parts hierarchically, such that we list out articulated parts and independent affordance parts, if articulated parts have specific subparts that are related to interactions - we break down the articulated parts further into affordance parts.
% \todo{Describe the orientation procedure once implemented}
% While some of the datasets include the metric sizes of the shapes, some are not guaranteed (ShapeNet, Obajverse, TexVerse). For this matter, we design a heuristic that scales the objects into appropriate sizes by sampling from manually-defined, per-category ranges.
% The following modules use precomputed segmentation for processing. We employ SSTK to compute the segments using connectivity- and clustering-based segmentation algorithms. Connectivity-based segmentation grows the segments based on whether two triangles share the same vertex or have vertices within some very small thresholds. Whereas clustering-based algorithm grows the segments by comparing whether the normals of the neighboring triangles are similar enough. The reason behind having multiple segments is that connectivity segments can sometimes grow too large due to the poor mesh structure. Clustering is supplied as an alternative that, on contrary, tends to over-segment which is helpful in such cases. \Ali{explain why you need this and then explain how you do it.}
%  Finally, we render multi-view images using BlenderProc\footnote{\url{https://github.com/DLR-RM/BlenderProc}}, generating both RGB images and corresponding precomputed segmentation maps. The 16 viewpoints are sampled uniformly over the sphere, consistent for each object. This allows to provide a full coverage of the objects exterior which is crucial for segmentation step. }

\subsection{Part Segmentation}
As mentioned in \Cref{subsec: design_principles}, each object in Artiverse is decomposed into parts that are associated to articlation hierarchy and interaction affordance.
For every object category, human experts design a predefined template listing all possible part labels shared across instances within that category.
These templates may be refined during the human verification stage if additional parts are discovered in complex models.
Leveraging the template, our part annotation strategy follows a two-stage process: we first generate initial part proposals using learning-based models and geometric algorithms, and then refine them through human verification.

\mypara{Initial proposals.}
Our part labels are designed to be semantically meaningful.
However, unlike general semantic segmentation, the boundaries of our parts are determined by functional behavior rather than purely visual appearance, leading to subtle but critical distinctions.
Therefore, it is essential to employ a segmentation model that can incorporate our contextual definitions of each label, making off-the-shelf open-vocabulary segmentation models based purely on text prompts unsuitable for this task.
We adopt the adaptive image segmentation model ASIA~\cite{perla2025asia}, which supports few-shot customization of label semantics.
To train ASIA, we manually annotate a dozen representative models for each category and use them as few-shot exemplars on multi-view renderings.
The trained model produces dense, label-aware part predictions for new shapes, reflecting the semantic intent under our context.

\mypara{Map proposals to 3D part instances.}
To project 2D segmentation results back onto 3D meshes, we first pre-compute over-segments based on the mesh's topological connectivity.
Each over-segment aggregates label votes from multi-view projections according to the number of covered pixels.
Unlabeled internal surfaces are assigned part labels using a distance-based propagation that considers the physical proximity of sampled surface points.
Once semantic segmentation converges, part instances are decomposed from each semantic group.
We employ a union-find algorithm to obtain disjoint, intra-connected sets of mesh segments, each forming an independent part instance, determined by local geometric continuity and spatial distance.

\mypara{Human verification.}
At the end of the segmentation stage, human verification is required to check the accuracy of each part instance and the correspondnce to its part labels that are proposed by the automation process above. 
We develop web interface for annotators to check whether it requires correction, and correct any mistakes with 3D part annotation toolkit and refine the part labels if needed.
As the last step, human experts will verify the annotations from annotator to ensure clean and consistent part segmentation.

% \input{figures/preprocesing}


% \input{figures/segmentation}

% \di{As the data at our specific label granularity is not available and annotating a sufficient amount for supervised methods is expensive, we resort to the method that is capable to produce segmentation based on few-shot fine-tuning. Segmentation module is outlined in \Cref{fig:segmentation}.

% \Ali{When we use any model, specially, our own models, we should make it clear why we used it or make it a soft claim and say one can use any other technique that is for example few shot segmentation. This avoids negative comments about being biased. }ASIA takes multi-view images as input and produces the semantic segmentation maps. Starting with at least 5 manually annotated shapes, we fine-tune ASIA per-category on 16 views and then proceed to run inference on previously rendered views of all shapes in the respective categories. The fine-tuning shapes are obtained by either remapping the labels from PartNet-Mobility dataset are annotating a few shapes manually from the data selected for Artiverse.

% The segmentation is propagated onto mesh using precomputed segments and corresponding renderings. For each view, we iterate over each visible segment and record what semantic labels and their pixel counts that were assigned to this segment. Afterwards, we simply pick the label with the largest pixel count to be a label of a particular segment. Now, there are two remaining steps - assigning semantic labels to occluded segments and clustering the segments into instances \todo{use parts instead of instances?}.

% In order to resolve the labels for occluded segments, we start by sampling 100k points from the object, recording the indices of segments the points are sampled from. For each occluded segment, we find the closest point from the point cloud subset of segments that have labels and select the label of corresponding segment.

% We employ similar strategy to obtain separate instances. Using a point cloud with 100k points, we sequentially process sub-point-clouds for each semantic label. In such sub-point-cloud, we iterate over every pair of segments and compute the shortest distance between the points of two segments. As this step involves only two segments at a time - it is parallelizable, mitigating potentially large number of pairs. We consider a pair of segments connected if the distance between them is less than a threshold. Finally, we use union-find algorithm to obtain disjoint intra-connected sets of segments that become separate part instances.

% \mypara{Segmentation Correction.} As segmentation proposals can be imperfect, we do a pass of correcting the segmentation manually. Each shape with the segmentation proposal loaded is presented in the custom UI that embeds SSTK's Part Annotator Interface. In this 3D viewer, annotators can observe and correct segmentation if needed, while the UI records which shapes have been already processed. If the correction is required, the part annotator allows selecting the whole segment rather than individual triangles akin to our propagation procedure, hence making it more efficient.

% \mypara{Segmentation Verification. } In order to eliminate human error factor fully and guarantee clean segmentation, we perform a second pass over the annotations, using a separate UI. In this UI, annotators are presented with a turntable video with a view revolving around each part of the object. The part of interest is highlighted with bright material and other parts are assigned semi-transparent gray material \Ali{A nice figure might be useful.}. This allows to quickly assess the quality of the segmentation within the context of the object's neighboring parts. If any changes are required, the annotator can open the correction UI and implement them. 

\subsection{Interior Completion}
For some categories, such as appliances and furnitures, interior serves as critical structure to enable their full functionality,
However, a significant portion of objects in our data source (e.g., ShapeNet, Objaverse, 3D-Future) lack sufficiently detailed interior geometry.
To provide assets that behave realistically in physical simulation, we complete the interiors of these objects where necessary.
We focus on three types of interiors in completion as described below.

\mypara{Partial articulated parts.}
Some articulated parts are partially modeled, with interior geometry omitted because it is not visible when the part is in their resting state.
This issue is typical for components exhibiting translational motion, where hidden regions are revealed only during articulation.
For example, many drawers are modeled with only the front panel, while the inner box is missing.
We design geometric-informed completion algorithm for such parts, extending the geometry consistently with the motion constraints to ensure plausibility in full motion range.

\mypara{Missing articulated parts.}
Certain appliances contain movable internal components that are entirely absent in many 3D assets.
Examples include dishwashers with baskets for dishes, microwaves with rotating turntables, and refrigerators with movable storage compartments.
To address this, we implement procedural algorithms that populate these missing elements by referencing similar parts from other objects within the same category, ensuring functional completeness and structural realism.

\mypara{Missing affordance part.}
Furniture and appliance bodies that provide storage space are often modeled as hollow shells, resulting in unrealistic behavior when interacting with other objects.
To restore functional realism, we add interior affordance structures such as shelves, racks, and dividers that correspond to the intended use of the object, e.g., refrigerator shelves for food placement or wardrobe racks for hanging clothes.
These interior completions are generated procedurally following category-specific templates that ensure geometric consistency and plausible spatial layout.


% \subsection{Interior Completion}

% \input{figures/interior_completion}

% \di{We distinguish multiple types of interior completion: articulated part completion, articulated part addition, base part completion. For each type, we determine the set of categories commonly requiring interior completion and design a set of heuristics, outlined in \Cref{fig:int_comp}.

% \mypara{Articulated part completion.} This case is concerned with articulated parts that have only the partial geometry present and when it is crucial for the interactivity of the object. We identify one instance of this type - drawers. The geometry behind the front panel is typically missing from drawers in the static datasets. We leverage the heuristic from the prior work~\cite{iliash2024s2o} that infers the drawer box by shooting rays behind the drawer's front panel and populating the box panels based on ray intersections.

% \mypara{Articulated part addition.} This completion type is used in large appliances that are usually modelled without interior articulated parts in static datasets, which are crucial for the object's interactivity. We begin by identifying a set of categories which require such type of completion and proceed to annotate them with segmentation \Ali{provide an example}. Our assumption is that in some of the cases the interiors actually will be present, so we can use the segmented parts obtained upstream to populate the empty objects, with corresponding articulations. \todo{Describe the retrieval procedure once implemented. }


% \mypara{Base part completion.} In some cases, the base part needs to be completed to obtain fully-functional object. This is especially prominent in multiple types of furniture, where the interiors behind the doors are commonly not modelled in static datasets. In particular, we target adding shelves and clothing rails to the appropriate furniture categories. We begin by determining whether the models already have interiors by checking the segmentation form the preceding module. If the model has no interiors, we employ a set of heuristics that procedurally generate the interiors based on model's geometry. \todo{Describe in detail for the supplement. }

% \mypara{Verification.} The completed interiors are verified together with articulations during the motion verification stage. \todo{The correction of completed interiors is not really an option currently, we can do it manually, however.}

% }

\subsection{Motion Annotation}
At this stage, models already contain verified part segmentations and complete geometric structures, including interiors where applicable.
We follow a similar strategy as in part segmentation, where automated motion proposals are first generated and later verified by human experts to ensure accuracy and physical plausibility. 

\mypara{Initial proposal.}
We first prompt VLMs to leverage their visual understanding capabilities to identify the motion type when it cannot be uniquely determined from the part labels.
Kinematic dependencies between articulated parts are then inferred based on spatial connectivity and dependency options defined in the per-category templates.
Then we design algorithms to predict the joint parameters, including axis origin. direction and joint limit.
In particular, we establish general rules that utilize the PCA-aligned oriented bounding boxes of parts and sampled points around the contact region to infer motion parameters for different motion types, constrained by geometric contact and collision relationships.
These inference rules are reusable across categories and are registered for different part types, requiring only minor adjustments for specialized components.

\mypara{Human verification.}
In motion verification stage, human annotators validate two key aspects: 1) whether the completed interior geometry is realistic, and 2) whether the proposed motions are physically plausible.
We develop a web-based interface that enables annotators to visualize and adjust articulation behavior interactively, modify joint parameters, and edit kinematic graphs as needed.
To improve efficiency, the interface supports features such as motion copying between similar parts and instant motion previews, allowing rapid correction and validation of proposed motion parameters.

% \input{figures/articulation}

% \di{Once clean segmentation is available, we proceed to annotate the articulations of the parts. Here, we once again, employ semi-automated process such that the proposals \Ali{Articulation proposals? How do they look like? Not clear here specially without fig} are automatically produced and later are corrected and verified by human annotators. The outline of the model can be seen in \Cref{fig:articulation}.

% \mypara{Motion Proposals.} We develop a set of heuristics that are used to create articulation proposals \Ali{Don't keep reminding the readers that you are using heuristic.}. In attempt to create a general framework, we leverage two facts: motion of many parts can be inferred from high-level geometrical cues such as centroids and bounding boxes \Ali{centroid and BBs of what? the whole object or the parts?}, motion of some parts is also influenced by where those connect to their parents. We develop custom heuristics for the parts that do not fall into this framework.

% As bounding boxes are crucial for these heuristics, we must ensure their quality. To this end, we compute three types of bounding boxes and select the best one. The types of bounding boxes are: 1) \texttt{AABB} - simple axis-aligned bounding box obtained from minimum and maximum points of the parts 2) \texttt{POBB} - oriented bounding box obtained by PCA analysis of the point cloud sampled uniformly for the part, such that principal axes are normals of the bounding box faces 3) \texttt{GOBB} - gravity-aligned oriented bounding box that is designed to respect the gravity explicitly, with face normals for non-vertical dimensions obtained from PCA analysis of the points projected onto XZ (horizontal) plane \Ali{on the second read, specially this part need clarifications and ustifications that why this is needed and useful}. The best bounding box is pre-determined for some parts, for others - we employ a heuristic that selects the best bounding box based on the volume, so that the bounding box with the smallest volume is considered the best. However, if \texttt{GOBB} is second-best and is within 5\% of volume of the smallest-volume bounding box - we pick it instead. This is done to prevent the cases where \texttt{POBB} fits a tighter, but less natural bounding box \Ali{ show such a case}. \Ali{Needs a visualization. It is hard to exactly know what is going on. Here, the best means tightest? if bot, what are the other criteria?}

% We begin by inferring joint type for each part. Leveraging the templates, the trivial case is if the part has a single joint type. In other cases, we employ heuristics to resolve motion types. \Ali{Too many reference to heuristic. You should use heuristic when it is not too relaibel. Otherwise, you can say a reliable algorithm or procedure.}

% For axis and origin, there are 4 simple heuristics that can be used for the total of \todo{xxx} parts across \todo{xxx} categories: 1) \texttt{longprism} - prismatic joint with axis along the longest dimension of the bounding box 2) \texttt{orthoprism} - prismatic joint with axis orthogonal to the largest face of the bbox 3) \texttt{centerupcont} - continuous joint with axis pointing upwards and pivot being the part's centroid 4) \texttt{centerorthocont} - continuous joint with axis orthogonal to the largest face of the bounding box and centroid as a pivot. These, combined with occasional per-category rules, allow us to process \todo{xxx}\% of parts. \Ali{A fig is needed to explain. You should also gibve stats that for X\% of objects such a heuristic will just work becuase most of the parts are moved along the longest dimension of their BB. If space is an issue, shorten here and refer readers to the supp mat. }

% Some of the parts that exhibit rotation might have axis that is straightforward to obtain either by hard-coding or leveraging one of the 4 heuristics above. However, origins might be not as straightforward as centroids. We, however, notice that in many such cases the origin can be inferred from the centroids of areas where the part of interest connects to parent (i.e., where casters connect to the star base of the office chair). For this matter, we leverage the part connectivity graph available from the segmentation module. We find where the parts connect by sampling the points from both parts and finding the closest 5\% of points from child part to parent part. Then, we use these 5\% of points as a guidance to re-fit the bounding box around the local connection region \Ali{Figure}. Rather than computing the optimal bounding box, we construct it by translating the sides of the bounding box that was defined for the child part also ensuring that the volume of this bounding box is at least 5\% of the volume of the full bounding box, ensuring proper coverage of the region. Finally, we compute centroid of the points that fall into this local bounding box, setting it as a motion origin.

% \input{figures/articulation_ranges}

% Finally, we need to infer motion ranges. For some parts, motion ranges are trivial (i.e., doors) assuming the part is always in a fixed state \Ali{Why are doors trivial?}. While true for some parts, others can be in arbitrary poses. In addition, some of the parts can be arbitrarily constrained by the neighboring geometry, preventing from using simple hard-coded values. These challenges are visualized in \Cref{fig:articulation_ranges}. To this end, we propose collision- and detachment-driven heuristics. Here we use trimesh\footnote{\url{https://trimesh.org/}} to measure the presence and number of collision points. For joints exhibiting rotation, we run a simulation of the joint movement with motion parameters inferred previously. Our goal is to determine how much part needs to be rotated to collide with other geometry of the object. At each step, we move the part according to its parameters and measure the number of collision points. As our source shapes were not designed with being articulated in mind, parts might already exhibit some collisions in the resting state. To this end, we rather rely on the relative increase of number of collision points between previous and current timestep. In particular, in order to classify the event as a collision, we must observe a sustained increase in collision points over several steps, followed by a significant drop. Specifically, we require the number of collisions to rise for a few steps and to exceed the initial collision count by some factor. If such a ramp-to-peak pattern is detected, we classify the event as a meaningful collision and terminate the simulation. We repeat the process in other direction to obtain second collision bound. Then, depending on the part and category, these bounds can be used as motion ranges either directly by taking a safe subrange (i.e., 80\% of the collision-to-collision range) or combined with some hard-coded values refining them. For prismatic joints, we first measure detachment distance. We begin by offsetting the part in a random direction to ensure the collision in the resting state, then we proceed to run similar simulation but now we rather look for the event of collisions disappearing. Once detachment range is established, we start the simulation in other direction now looking for the collision boundary. Finally, these detachment-collision bounds are per-category processed and are used as motion range proposals. \Ali{This is too long and tedious to read. I am not sure anybody is interested and can read all these details. You need to significantly reduce the text here as all you are doing is essentially simulating the movement and checking any collision with other parts. These all need to move to supp mat. }

% \input{figures/articulation_heuristics}

% Examples of articulation heuristics applied can be seen in \Cref{fig:articulation_heuristics}.} \Ali{no new paragraph.}

% \mypara{Kinematic Graph. } Finally, we compute the graph of how parts are connected which later, combined with articulations, serves as a kinematic graph. For this matter, we iterate over each part and lookup which are potential parents of this part in the template \Ali{Did we mention/define template before?}. Then, we use points to compute the distances between parts similarly to the previous steps and find the closest part such that its label is in the list of potential parents and set it to be a parent of the part of interest.  After processing all the parts this way, the graph is complete.}

% \di{
% \mypara{Motion correction.} Analogously to segmentation, articulation annotations also undergo motion correction in a similar user interface, with an embedded SSTK motion correction window. In this interface, users can manually play the motion of each part and modify each aspect of the articulation annotation accordingly.
% }

% \di{
% \mypara{Motion verification. } Motion verification interface is similar to segmentation verification one. Here, instead of turntables, we render similar videos with highlighted parts but now articulating. As this is the last interface where the annotators manually check the objects, some of the submodules described next also use it to verify their outputs. For instance, interior completion results and inferred material labels are verified here as discussed later.
% }

\subsection{Physical Properties}
To improve the realism of the simulation of the resulting assets, we enrich the objects with masses. 
Computing the mass consists of three steps: computing the volume of the part, inferring the material label and finally retrieving the density.

\mypara{Volume computation.} 
Volume is ill-defined for frequently non-watertight objects we are working with. 
Hence, we preprocess the geometry of each part to be watertight first and then compute its volume. 

\mypara{Inferring density.}
To estimate part density, we first infer its material label using VLMs.
We assume material consistency across repeated parts and inheritance from base components when applicable, which reduces redundant inference.
For parts requiring material prediction, we render two close-up views—one highlighting the part and one showing original textures—and prompt the VLM to select the most mass-relevant material from predefined candidates per category.
This ensures robust mass estimation even when exterior and interior materials differ.
The final part mass is computed by multiplying the estimated density with the part volume.

% \di{
% \subsection{Physical Parameters}

% To improve the realism of the simulation of the resulting assets, we enrich the objects with masses. Computing the mass consists of three steps: computing the volume of the part, inferring the material label and finally retrieving the density.

% \mypara{Volume computation.} Volume is ill-defined for frequently non-watertight objects we are working with. Hence, we preprocess the geometry of each part to be watertight first and then compute its volume. \todo{Note, this is a preliminary version; more robust computation is under development}

% \mypara{Inferring the density.} In order to infer the density, we first need to obtain the material label. Moreover, we notice that: 1) For many parts, multiple instances of the same part in a single object have the same material; 2) Some parts consistently inherit the material of the base part. These observations lead to the design of a few processing strategies to save the compute, with the one being used specified for each part of each category. If the part was determined to require inference of the material label, we begin by rendering two views new image from the view slightly zoomed-in on the part: one with part of interest being highlighted by the bright material and other part in semi-transparent gray to indicate the part of interest, and the other with original materials of the object. These images are concatenated and are passed to VLM, that is prompted to pick one of the possible materials that are specified for each part of each category. In particular, as we are interested in computation of mass, we prompt the VLM to pick the material that contributes the most to the mass of the part. This way, the cases where the exterior and interior materials of the part are different do not corrupt the computation of the mass. The material labels are verified during the motion verification by displaying the textured rendering of the part and the inferred material. Finally, we multiply the volume of each part by density to obtain the mass of each part in kilograms. \Ali{Again this is too long. Essentially, you are assuming consistency among the material of the parts and ask VLM to measure physical parameters. Details can go to supp mat. }
% }

==> tables/pipeline_stats.tex <==
\begin{table}[t]
    \centering
    \resizebox{\linewidth}{!}{
    \begin{tabular}{@{}lll@{}}
    \toprule
    Submodule & Step & Statistics \\
    \midrule
    \multirow{1}{*}{Preprocessing} & - & Time per shape (m): $N \pm std$ \\
    \midrule
    \multirow{6}{*}{Segmentation} & Obtaining proposals & Time per shape (m): $N \pm std$\\ \cmidrule{2-3}
                                  & \multirow{2}{*}{Correction} & Time per shape (m): $N \pm std$ \\
                                                            &    & Shapes requiring no correction: $N$ \\ \cmidrule{2-3}
                                    
                                  & \multirow{2}{*}{Verification} & Time per shape (m): $N \pm std$ \\
                                                             &     & Shapes sent back for correction: $N$ \\
    \midrule
    \multirow{6}{*}{Articulation} & Obtaining proposals & Time per shape (m): $N \pm std$\\ \cmidrule{2-3}
                                  & \multirow{2}{*}{Correction} & Time per shape (m): $N \pm std$ \\
                                                            &    & Shapes requiring no correction: $N$ \\ \cmidrule{2-3}
                                    
                                  & \multirow{2}{*}{Verification} & Time per shape (m): $N \pm std$ \\
                                                             &     & Shapes sent back for correction: $N$ \\
    \midrule
    \multirow{1}{*}{Interior Completion} & - & Time per shape (m): $N \pm std$ \\
    \midrule
    \multirow{1}{*}{Physical Parameters} & - & Time per shape (m): $N \pm std$ \\
    
    \bottomrule                                 
    
    \end{tabular}
    }
    \caption{Pipeline inference statistics.}
    \label{tab:pipeline_stats}
\end{table}

==> tables/pipeline_stats_new.tex <==
\begin{table}[t]
    \centering
    \resizebox{\linewidth}{!}{
    \begin{tabular}{@{}lll@{}}
    \toprule
    Submodule & Step & Statistics \\
    \midrule
    \multirow{4}{*}{Segmentation}  
                                  & \multirow{2}{*}{Correction} & Time per shape (m): $81.7 \pm 102.0$ \\
                                                            &    & Shapes requiring no correction: $698(16.0\%)$ \\ \cmidrule{2-3}
                                    
                                  & \multirow{2}{*}{Verification} & Time per shape (m): $81.6 \pm 103.9$ \\
                                                             &     & Shapes sent back for correction: $872(22.8\%)$ \\
    \midrule
    \multirow{2}{*}{Articulation} 
                                  & \multirow{2}{*}{Correction} & Time per shape (m): $55.8 \pm 88.7$ \\
                                                            &    & Shapes requiring no correction: $0(0\%)$ \\
    \bottomrule                               
    
    \end{tabular}
    }
    \caption{Manual Annotation Statistics.}
    \label{tab:pipeline_stats}
\end{table}

==> tables/quant_segment_s2o.tex <==
\begin{table}[t]
\centering
{
\begin{tabular}{@{} l rrr rrr @{}}
\toprule
& \multicolumn{3}{c}{Micro} & \multicolumn{3}{c}{Macro} \\
\cmidrule(l{0pt}r{2pt}){2-4} \cmidrule(l{0pt}r{2pt}){5-7}
Method & P & R & F1 & P & R & F1 \\
\midrule
ASIA (few-shot)\\
ASIA (extended) \\
FPNGroup (full) \\
\bottomrule
\end{tabular}
\caption{Mesh segmentation comparison. ASIA few-shot, original setup using at least 5 examples and reuses some of the data from PartNet-Mobility, ASIA extended that uses at least 10 examples all coming fromo Artiverse, FPNGroup trained on full Artiverse-train.
}
}
\label{tab:quant_segment_s2o}
\end{table}

==> tables/user_study.tex <==
\begin{table}[t]
    \centering
    \resizebox{\linewidth}{!}{
    \begin{tabular}{@{}lccc@{}}
    \toprule
    & PartNet-Mobility & Artiverse-auto & Artiverse-semi-auto \\
    \cmidrule{2-4}

    Avg Rank & - & - & - \\

    \bottomrule                                 
    
    \end{tabular}
    }
    \caption{Shape annotation quality user study results.}
    \label{tab:user_study}
\end{table}
